Two-player Knock 'em Down

We analyze the two-player game of Knock 'em Down, asymptotically as the number of tokens to be knocked down becomes large. Optimal play requires mixed strategies with deviations of order sqrt(n) from the naive law-of-large numbers allocation. Upon rescaling by sqrt(n) and sending n to infinity, we show that optimal play's random deviations always have bounded support and have marginal distributions that are absolutely continuous with respect to Lebesgue measure.

==> ejplogo.tex <==
{%
    \centerline {%
        \hbox {%
            %\large
            \vrule  height -0.4 pt depth 0.8 pt width 26.5 em\space %
            \kern  - 26.5 em\space %
            \raise   0.03ex  \hbox {\bf  E}\space %
            \raise   0.06ex \hbox {l}\space %
            \raise  .13ex \hbox {e}\space %
            \raise  .24ex \hbox {c}\space %
            \raise  .45ex \hbox {t}\space %
            \raise  .78ex \hbox {r}\space %
            \raise  1.31ex \hbox {o}\space %
            \raise  2.08ex \hbox {n}\space %
            \raise  3.14ex \hbox {i}\space %
            \raise  4.53ex \hbox {c}\space %
            \kern    1em\space %
            \raise  8.15ex \hbox {\bf  J}\space %
            \raise  10.15ex \hbox {o}\space %
            \raise  12.04ex \hbox {u}\space %
            \raise  13.60ex \hbox {r}\space %
            \raise  14.64ex \hbox {n}\space %
            \kern  .3 em\space %
%OLD        \vrule \space %
%BETTER     \vrule  height 14.5ex \space %
            \vrule  depth 0.8pt height 14.5ex \space % %BEST!
            \kern  -.3em\space %
            \raise  15ex \hbox {a}\space %
            \raise  14.64ex \hbox {l}\space %
            \kern    1em\space %
            \raise  12.04ex \hbox {o}\space %
            \raise  10.15ex \hbox {f}\space %
            \kern    1em\space %
            \raise  6.23ex \hbox {\bf  P}\space %
            \raise  4.53ex \hbox {r}\space %
            \raise  3.14ex \hbox {o}\space %
            \raise  2.08ex \hbox {b}\space %
            \raise  1.31ex \hbox {a}\space %
            \raise  .78ex \hbox {b}\space %
            \raise  .45ex \hbox {i}\space %
            \raise  .24ex \hbox {l}\space %
            \raise  .13ex \hbox {i}\space %
            \raise  .06ex \hbox {t}\space %
            \raise  .03ex \hbox {y}%
            }%
       }%
}%
%

